Territorial differences in the spread of COVID-19 in European regions and US counties

This article explores the territorial differences in the onset and spread of COVID-19 and the excess mortality associated with the pandemic, across the European NUTS3 regions and US counties. Both in Europe and in the US, the pandemic arrived earlier and recorded higher Rt values in urban regions than in intermediate and rural ones. A similar gap is also found in the data on excess mortality. In the weeks during the first phase of the pandemic, urban regions in EU countries experienced excess mortality of up to 68pp more than rural ones. We show that, during the initial days of the pandemic, territorial differences in Rt by the degree of urbanisation can be largely explained by the level of internal, inbound and outbound mobility. The differences in the spread of COVID-19 by rural-urban typology and the role of mobility are less clear during the second wave. This could be linked to the fact that the infection is widespread across territories, to changes in mobility patterns during the summer period as well as to the different containment measures which reverse the causality between mobility and Rt.

==> Table3.tex <==
{\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{7}{c}{Rt first wave} \\ 
\cline{2-8} 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 Internal -3 & 0.540$^{***}$ &  &  &  &  &  &  \\ 
  & (0.107) &  &  &  &  &  &  \\ 
  Internal -2 &  & 0.888$^{***}$ &  &  &  &  &  \\ 
  &  & (0.162) &  &  &  &  &  \\ 
  Internal -1 &  &  & 1.580$^{***}$ &  &  &  &  \\ 
  &  &  & (0.198) &  &  &  &  \\ 
  Internal &  &  &  & 1.839$^{***}$ &  &  &  \\ 
  &  &  &  & (0.220) &  &  &  \\ 
  Internal +1 &  &  &  &  & 1.640$^{***}$ &  &  \\ 
  &  &  &  &  & (0.241) &  &  \\ 
  Internal +2 &  &  &  &  &  & 1.069$^{***}$ &  \\ 
  &  &  &  &  &  & (0.264) &  \\ 
  Internal +3 &  &  &  &  &  &  & 0.554$^{**}$ \\ 
  &  &  &  &  &  &  & (0.276) \\ 
 \hline \\[-1.8ex] 
Observations & 3,034 & 3,374 & 3,528 & 3,572 & 3,567 & 3,559 & 3,553 \\ 
R$^{2}$ & 0.143 & 0.026 & 0.030 & 0.033 & 0.026 & 0.018 & 0.015 \\ 
Adjusted R$^{2}$ & 0.141 & 0.024 & 0.028 & 0.031 & 0.024 & 0.016 & 0.013 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
}

==> Table4.tex <==
{\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{7}{c}{Rt second wave} \\ 
\cline{2-8} 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 Internal -3 & $-$0.040$^{***}$ &  &  &  &  &  &  \\ 
  & (0.006) &  &  &  &  &  &  \\ 
  Internal -2 &  & $-$0.043$^{***}$ &  &  &  &  &  \\ 
  &  & (0.006) &  &  &  &  &  \\ 
  Internal -1 &  &  & $-$0.045$^{***}$ &  &  &  &  \\ 
  &  &  & (0.006) &  &  &  &  \\ 
  Internal &  &  &  & $-$0.046$^{***}$ &  &  &  \\ 
  &  &  &  & (0.006) &  &  &  \\ 
  Internal +1 &  &  &  &  & $-$0.050$^{***}$ &  &  \\ 
  &  &  &  &  & (0.006) &  &  \\ 
  Internal +2 &  &  &  &  &  & $-$0.054$^{***}$ &  \\ 
  &  &  &  &  &  & (0.007) &  \\ 
  Internal +3 &  &  &  &  &  &  & $-$0.056$^{***}$ \\ 
  &  &  &  &  &  &  & (0.007) \\ 
 \hline \\[-1.8ex] 
Observations & 10,539 & 10,541 & 10,542 & 10,542 & 9,991 & 9,444 & 8,899 \\ 
R$^{2}$ & 0.035 & 0.036 & 0.036 & 0.036 & 0.039 & 0.042 & 0.045 \\ 
Adjusted R$^{2}$ & 0.035 & 0.035 & 0.035 & 0.036 & 0.038 & 0.041 & 0.044 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
}

